A PoW-less Bitcoin with Certified Byzantine Consensus

Distributed Ledger Technologies (DLTs), when managed by a few trusted validators, require most but not all of the machinery available in public DLTs. In this work, we explore one possible way to profit from this state of affairs. We devise a combination of a modified Practical Byzantine Fault Tolerant (PBFT) protocol and a revised Flexible Round-Optimized Schnorr Threshold Signatures (FROST) scheme, and then we inject the resulting proof-of-authority consensus algorithm into Bitcoin (chosen for the reliability, openness, and liveliness it brings in), replacing its PoW machinery. The combined protocol may operate as a modern, safe foundation for digital payment systems and Central Bank Digital Currencies (CBDC).

==> ccs-keywords.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10011007.10010940.10010971.10011120</concept_id>
       <concept_desc>Software and its engineering~Distributed systems organizing principles</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978</concept_id>
       <concept_desc>Security and privacy</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Software and its engineering~Distributed systems organizing principles}
\ccsdesc[500]{Security and privacy}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Bitcoin, blockchain, distributed ledger, Byzantine consensus, threshold signature scheme}

